Temperature states in Powder Bed Fusion additive manufacturing are structurally controllable and observable

Powder Bed Fusion (PBF) is a type of Additive Manufacturing (AM) technology that builds parts in a layer-by-layer fashion out of a bed of metal powder via the selective melting action of a laser or electron beam heat source. The technology has become widespread, however the demand is growing for closed loop process monitoring and control in PBF systems to replace the open loop architectures that exist today. Controls-based models have potential to satisfy this demand by utilizing computationally tractable, simplified models while also decreasing the error associated with these models. This paper introduces a controls theoretic analysis of the PBF process, demonstrating models of PBF that are asymptotically stable, stabilizable, and detectable. We show that linear models of PBF are structurally controllable and structurally observable, provided that any portion of the build is exposed to the energy source and measurement, we provide conditions for which time-invariant PBF models are classically controllable/observable, and we demonstrate energy requirements for performing state estimation and control for time-invariant systems. This paper therefore presents the foundation for an effective means of realizing closed loop PBF quality control.

==> abstract.tex <==
\begin{abstract}
% Powder Bed Fusion (PBF) is a type of Additive Manufacturing (AM) technology that builds parts in a layer-by-layer fashion out of a bed of metal powder via the selective melting action of a laser or electron beam heat source.  The technology has become widespread, however the demand is growing for closed loop process monitoring and control in PBF systems to replace the open loop architectures that exist today.  This paper presents a novel modeling strategy for the PBF process which incorporates established controls techniques with a simplified FEM-based conductive model of PBF thermal physics in order to obtain accurate models without incurring high computational burden.  This study shows that systems designed according to this strategy are controllable and observable despite uncertainty in parameter values for most system geometries, that such systems can be implemented in digital controls techniques without incurring loss of controllability/observability, and demonstrates the efficacy of using state estimators to improve model accuracy.  The significant outcomes of this study are exploring the feasibility limits of this approach and demonstrating its effectiveness in simulation.

% Powder Bed Fusion (PBF) is a type of Additive Manufacturing (AM) technology that builds parts in a layer-by-layer fashion out of a bed of metal powder via the selective melting action of a laser or electron beam heat source.  The technology has become widespread, however the demand is growing for closed loop process monitoring and control in PBF systems to replace the open loop architectures that exist today.  This paper presents a novel modeling strategy for the PBF process that expresses a simplified heat conduction model of the governing thermal physics as an LTI state space system.  This study shows that systems designed according to this strategy are asymptotically stable, stabilizable, and detectable, and furthermore that they are controllable and observable despite uncertainty in parameter values for most system geometries.  This model architecture is amenable to closed-loop process monitoring and control strategies, which provide accurate results for comparatively little computational burden.  This paper therefore presents the foundation for an effective means of realizing closed loop PBF process monitoring.

Powder Bed Fusion (PBF) is a type of Additive Manufacturing (AM) process that builds parts in a layer-by-layer fashion out of a bed of metal powder via selective melting of powder by a laser or electron beam heat source.  Research interest in PBF continues to grow, as is demand for closed loop process monitoring and control in PBF systems to replace the open loop architectures that exist today. This paper contains a controls theoretic analysis of the Powder Bed Fusion (PBF) process, demonstrating the basic properties that PBF is asymptotically stable, stabilizable, detectable, structurally controllable and structurally observable, provided that any portion of the build is exposed to the energy source and measurement.  These properties are shown to hold in both time-invariant and time-varying models.  We provide conditions for the classical controllability and observability of time-invariant PBF models.  These conditions reveal when certain PBF systems may have their thermal history be arbitrarily manipulated through their process inputs and estimated to arbitrary accuracy through measured process outputs.  Furthermore, we measure the expended actuator energy and absorbed sensor energy to accomplish such control and estimation under our framework.  Controls-based models have potential to satisfy this demand by utilizing computationally tractable, simplified models while also decreasing the error associated with these models.  This paper therefore presents the foundation for an effective means of realizing closed loop PBF process monitoring.  
\end{abstract}



==> cont_obs.tex <==
\section{Controllability and Observability}\label{sec:Controllability and Observability}
% \subsection{Controllability and Observability definitions}
% Linearizing the Hammerstein model outlined in Section \ref{sec:thermal_model} produces equations in the form of standard LTI state space systems.  As such, we utilize the well-known textbook definitions of controllability and observability in our analysis.    

% As in \cite{Wood_2018}, we continue to use that standard definition of observability detailed in \cite{chen_1999} and others: Thermal Model \eqref{eq: LTI_System} is ``said to be observable if for any unknown initial state $\mathbf{t}(0)$, there exists a finite $t_1>0$ such that knowledge of the input $\mathbf{u}$ and the output $\mathbf{y}$ over $[0,t_1]$ suffices to determine uniquely the initial stat $\mathbf{t}(0)$''.  To verify that this property holds, we leverage the rank test of the observability matrix $\mathcal{O}$.  As stated in \cite{chen_1999}, the pair $\left(\mathbf{A}, \mathbf{C}\right)$ is observable if 

% \begin{equation}
% \mathcal{O}=\left[\begin{array}{c}
% \mathbf{C}\\
% \mathbf{CA}\\
% \vdots\\
% \mathbf{CA}^{n-1}\\
% \end{array}
% \right]
% \end{equation}

% has rank $n$.  Similarly, when considering the linearized Hammerstein model, we use the standard definition for controllability given by \cite{Antasaklis_2007}: Thermal Model \eqref{eq: LTI_System} is ``said to be controllable if there exists an input that transfers the state from some initial condition $\mathbf{t}_0$ to the zero state in a finite time interval $\left[0,t_1\right]$, $t_1>0$.'' As with observability, we leverage the rank test of the controllability matrix $\mathcal{C}$.  As stated in \cite{Antasaklis_2007}, the pair $\left(\mathbf{A},\mathbf{B} \right)$ is controllable if

% \begin{equation}
% \mathcal{C}=\begin{bmatrix}
% \mathbf{B} & \mathbf{AB} & \dots & \mathbf{A}^{n-1}\mathbf{B}
% \end{bmatrix}
% \end{equation}

% has rank $n$.      


% \subsection{Network control theory: structural controllability}
% We analyze the controllability and observability of Thermal Model \eqref{eq: LTI_System} within the framework of \emph{structural} controllability and observability.  Our treatment of these concepts follows the presentation given in \cite{Liu_YY_2011} and is meant to be a brief introduction to the topic.  Readers interested in a more complete description of the subject should consult \cite{Liu_YY_2011}.\par 

% The theory of structural controllability/observability treats Thermal Model \eqref{eq: LTI_System} as a directed network of nodes and edges.  Interpreting Thermal Model \eqref{eq: LTI_System} this way is natural given that FEM discretizes domain $V$ into a set of nodes connected by edges and collected into elements. Fig. \ref{fig: StructuralControllability}(a)-(b) demonstrates this interpretation.  
% In keeping with the notation of \cite{Liu_YY_2011}, we refer to the network constructed by Thermal Model \eqref{eq: LTI_System} as $G(\mathbf{A})$.  

% Analysis of $G(\mathbf{A})$ via structural controllability/observability begins by assuming that the nonzero values of $\mathbf{A}$ and $\mathbf{B}$ are uncertain.  Assumption \textbf{A5}, in which material properties and heat input parameters were assumed uncertain, reflects this assumption. Our approach first assesses the structural controllability of Thermal Model \eqref{eq: LTI_System} and then assesses structural observability under the same framework. We supply the definition of structural controllability as given in \cite{Liu_YY_2011} below.

% \begin{defn}
% Thermal Model \eqref{eq: LTI_System} is \emph{structurally controllable} if the uncertain nonzero (free) parameters of $\mathbf{A}$ and $\mathbf{B}$ may be chosen such that the resultant system $(\mathbf{A,B})$ is controllable in the sense of Section \ref{sec:Controllability and Observability}A. 
% \end{defn} 
%  The notions of structural controllability abstract the idea of controllability away from the particular construction of $\{ \mathbf{A,B} \}$, and instead presens it as inherent properties of the given network topology.  This is a powerful tool for assessing system controllability/observability in the face of uncertain model parameters wherein two different parameter estimations may result in the construction of pairs $\mathbf{A_0,B_0}\}$ and $\{\mathbf{A_1,B_1}\}$, in which the former is uncontrollable  whereas the latter is controllable despite the network topology remaining constant.  Furthermore, as \cite{Liu_YY_2011} state, controllability is a \emph{dense} set.  This property means that that if a certain model parameter estimation results in an uncontrollable pair $(\mathbf{A_0,B_0})$ then there exists a completely controllable pair $(\mathbf{A_1,B_1})$ resulting from a different estimation such that $||\mathbf{A_1-A_0}||<\epsilon$ and $||\mathbf{B_1-B_0}||<\epsilon$ for all $\epsilon>0$.  An infinitesimally small error in the estimated parameter values may produce a system $(\mathbf{A_1,B_1})$ that is controllable despite predictions of uncontrollability.  In posing the question of controllability as something inherent to the model structure rather than a consequence of specific parameter estimations, structural controllability removes this ambiguity. \par 

\subsection{Existence of perfect network matching}
The LTI structure of Case (1) allows us to leverage network theory tools for assessing structural controllability according to the definitions discussed in Section \ref{sec:Preliminaries}.  Doing so requires understanding the graph theory concept of a \emph{matching}, the definition of which is given below \cite{Liu_YY_2011}:
\begin{defn}
For a directed graph (digraph), a \emph{matching} is an edge set in the graph $G(\mathbf{A})$ in which no two edges share a common starting or ending vertex (node).  A vertex is \emph{matched} if it is an ending vertex of an edge in a matching.  Otherwise, it is \emph{unmatched}. A \emph{maximum matching} is any matching of $G(\mathbf{A})$ which has the maximum cardinality of all possible matchings.  A matching is \emph{perfect} if every vertex is matched.
\end{defn}
Fig. \ref{fig: StructuralControllability}C demonstrates the maximum matching corresponding to the network formed by a 3 node FEM mesh.  The edges constituting the matching are shown in red.  None of the edges share starting or ending vertices.  Crucially, the matching is formed from the edges corresponding to the self-loops within the network, and as such it is a perfect matching.
\begin{thm}\label{thm: Matching}
Any network formed from \eqref{eq:nonlinear_specific} contains a perfect matching.
\end{thm}
\emph{proof}: The $\mathbf{A}$ matrix which constructs the network $G(\mathbf{A})$ has the definition $\mathbf{A}=-\mathbf{M}^{-1}\mathbf{K}$, where $\mathbf{M}>0$, $\mathbf{K}>0$ and $\mathbf{M}$ is diagonal.   It follows from \cite{johnson_1970} that the diagonal elements of $\mathbf{K}$ and $\mathbf{M}$ are positive, and therefore that the diagonal elements of $\mathbf{A}$, $A_{ii}=-M^{-1}_{ii}K_{ii}$ are nonzero.  As such, every node in $G(\mathbf{A})$ always has a self-loop, and therefore a perfect matching may always be constructed from the self-loops within $G(\mathbf{A})$.  $\blacksquare$\par 

\subsection{Structural controllability/observability: LTI case}
We leverage Theorem 2 to define the structural controllability of Case (1) in terms of the number and location of network nodes that receive system input (driver nodes) and are observed to construct system output (observer nodes):\par 
\begin{thm}\label{thm: StructuralControllability}
Theorem 2 implies that Case (1) and Case (2) are structurally controllable provided that the FEM mesh contacts Face $\Omega$ of $V$.
\end{thm}
\emph{Proof}:  \cite{Liu_YY_2011} shows that if a perfect matching exists within $G(\mathbf{A})$, then the minimum number of driver nodes needed to control the system is one and that this node may be placed anywhere within the network.  As such, Theorem 2 implies that Case (1) is structurally controllable so long as a single driver node of the FEM mesh exists to receive input from the PBF laser beam. Case (1) is constructed assuming that the laser heat input falls on face $\Omega$ of $V$, and hence only the nodes laying on $\Omega$ are eligible to be driver nodes.  Therefore, if the FEM mesh contacts $\Omega$ then there must necessarily be at least one node that may be selected as a valid driver node of the system, and therefore the system is structurally controllable. $\blacksquare$\par 

The proof of structural controllability may be extended to show structural observability:\par 
\begin{thm}\label{thm: StructuralObservability}
Theorem \ref{thm: Matching} and Theorem \ref{thm: StructuralControllability} imply that Case (1) and Case (3) are structurally observable provided that the FEM mesh contacts Face $\Omega$ of $V$. 
\end{thm}
\emph{Proof}: The structural observability of $G(\mathbf{A})$ is equivalent to the structural controllability of $G(\mathbf{A}^\prime )$ \cite{Liu_YY_2013}.  Since all diagonal elements of $\mathbf{A}$ are nonzero, so too are those of $\mathbf{A}^\prime $ and hence Theorem \ref{thm: Matching} applies to $\mathbf{A}^\prime $.  Considering that Case (1) was constructed assuming that observer nodes exclusively lie on Face $\Omega$ of $V$, the rest of the proof follows similarly to that given for Theorem \ref{thm: StructuralControllability}.  

\subsection{Structural controllability/observability, LTV case}
We extend our conclusions of structural controllability/observability for LTI systems into the time-variant aspects of Cases (2), (3), and (4):

\begin{thm}\label{thm: LTI_Extension}
At any instant in time $t_0>0$ and provided that at least one node of $G(\mathbf{A})$ exists on $\Omega$, the networks constructed from Cases (3) and (4) are structurally controllable, and the networks constructed from Cases (2) and (4) are structurally observable.
\end{thm}
\emph{proof}:  The time-varying matrices $\mathbf{B}(t)$ and $\mathbf{C}(t)$ as defined in Sections \ref{sec:thermal_model}.3 and \ref{sec:thermal_model}.4 select the input and output nodes of the graph $G(\mathbf{A})$ at all instances in time and are smooth.  Therefore at any instant in time $t_0>0$, the graph $G(\mathbf{A})$ has at least one node selected as its input and its output, provided that at least one node on $\Omega$ exists, and therefore Theorems \ref{thm: StructuralControllability} and \ref{thm: StructuralObservability} may be applied to show that this network is both structurally controllable and observable. $\blacksquare$ 

Theorem 6 shows that Cases (2)-(4) are structurally controllable/observable at any instant in time.  We now wish to show that this property extends to structural controllability/observability over finite intervals of time, which measure the ability of these systems to be controlled through the input or observed through the input/output throughout nonzero time intervals, respectively.  To do so we first must show that the controllability and observability gramains over any finite time interval for Case (1) are positive definite:

\begin{thm}\label{thm: LTI_Gram_PD}
The controllability and observability Gramians defined by an LTI network with the structural properties of Case (1) are symmetric and positive definite over the time interval $0\leq t_0<t_1<\infty$, provided that the parameters that govern the nonzero values of $(\mathbf{A},
\mathbf{B},\mathbf{C})$ have been selected to render the structurally observable system observable.
\end{thm}
\emph{proof}:  We will show that the observability gramian is positive definite, with the proof for the controllability gramian proceeding similarly.  The observability gramian for an LTI system on the interval $\left[t_0,t_1\right]$ is defined as \cite{chen_1999}:

\begin{equation}\label{eq: LTI_Gram}
    W_{O,LTI}(t_0,t_1)=e^{-\mathbf{A}^\prime t_0}\left(\int_{t_0}^{t_1}\underbrace{e^{\mathbf{A}^\prime  t}\mathbf{C}^\prime \mathbf{C}e^{\mathbf{A}t}}_{\mathbf{P}(t)}dt\right)e^{-\mathbf{A}t_0}
\end{equation}

Consider the integrand term $\mathbf{P}(t)$ in \eqref{eq: LTI_Gram}. By \cite{Van_den_Bos_2007}, the product $\mathbf{C}^\prime\mathbf{C}$ is symmetric and positive semidefinite (PSD), denoted as $\mathbf{C}^\prime\mathbf{C}\geq0$.  By \cite{Horn_2013_LTV_cite}, this implies that the symmetric matrix product $\mathbf{P}(t)=e^{\mathbf{A}^\prime t}\mathbf{C}^\prime\mathbf{C}e^{\mathbf{A}t}=\left(e^{\mathbf{A}t}\right)^{\prime}(\mathbf{C}^{\prime}\mathbf{C})e^{\mathbf{A}t}\geq0$.  The integral term of \eqref{eq: LTI_Gram} may therefore be written as a Reimann Sum of symmetric PSD matrices:

\begin{equation}\label{eq: Reimann_Sum}
    I_{LTI}(t_0,t_1)=\int_{t_0}^{t_1}\mathbf{P}(t)dt=\lim_{||\Delta t||\to0}\sum_{k=1}^n\mathbf{P}(t^{*}_k)\Delta t_k
\end{equation}

In \eqref{eq: Reimann_Sum}, each $\Delta t_k$ represents the vanishing interval width and thus is positive.  Therefore by \cite{Horn_2013_LTV_cite}, the nonnegatively-weighted sum of $\mathbf{P}(t_k^{*})\geq0$.  Hence the symmetric $I_{LTI}(t_0,t_1)\geq0$ and therefore the symmetric product $W_{O,LTI}(t_0,t_1)=e^{-\mathbf{A}^\prime t_0}I_{LTI}(t_0,t_1)e^{-\mathbf{A}t_0}=\left(e^{-\mathbf{A} t_0}\right)^{\prime}I_{LTI}(t_0,t_1)e^{-\mathbf{A}t_0}\geq0$ \cite{Horn_2013_LTV_cite}.  However, by Theorem \ref{thm: StructuralObservability}, a given set of parameters governing the nonzero values of $(\mathbf{A},\mathbf{C})$ may be selected such that $(\mathbf{A},\mathbf{C})$ is observable by the definition of structural observability.  Hence a parameter set for $(\mathbf{A},\mathbf{C})$ exists such that $W_{O,LTI}(t_0,t_1)\geq0$ is nonsingular due to the fact that an observable LTI system is observable over any time interval \cite{chen_1999}.  The proof for a symmetric PD observability gramian is completed by acknowledging that a nonsingular symmetric PSD matrix is PD \cite{Horn_2013_LTV_cite}.  The proof showing a PD controllability gramian proceeds similarly under the definition of the controllability gramian given in \eqref{eq: LTI_Gram_Cont}\cite{chen_1999}. $\blacksquare$

\begin{equation}\label{eq: LTI_Gram_Cont}
    W_{C,LTI}(t_0,t_1)=e^{-\mathbf{A}t_0}\left(\int_{t_0}^{t_1}e^{\mathbf{A}t}\mathbf{B}\mathbf{B}^\prime e^{\mathbf{A}^\prime t}dt\right)e^{-\mathbf{A}^\prime t_0}
\end{equation}

We now extend Definition 3 to apply to time-varying Cases (2)-(4) over nonzero finite time intervals. These extensions are necessary because Cases (2)-(4) feature governing system parameters such as laser position that change with time and with uncertainty due to the inherent imprecision of the machine.  Definition 3 therefore is not applicable to assess structural controllability/observability over finite nonzero time intervals because it requires that the governing system parameters be fixed.  Our extension is as follows:

\begin{defn}
Denote the respective time-varying governing model parameters of Cases (2)-(4) as $\mathbf{p}(t)$. Cases (2)-(4) are \emph{structurally controllable} within the time interval $0\leq t_0<t_1<\infty$ if a $\mathbf{p}(t)$ exists such that the resultant system $(\mathbf{A},\mathbf{B}(t))$ is controllable in the sense of Section \ref{sec:Preliminaries}.1.  Similarly, Cases (2)-(4) are \emph{structurally observable} within the time interval $0\leq t_0<t_1<\infty$ if a $\mathbf{p}(t)$ exists such that the resultant system $(\mathbf{A},\mathbf{C}(t))$ is observable in the sense of Section \ref{sec:Preliminaries}.1.
\end{defn} 

Theorems \ref{thm: LTI_Extension} and \ref{thm: LTI_Gram_PD} allows us to show the structural observability of Cases (2) and (4) in the sense of Definition 5:

\begin{thm}\label{thm: LTV_Observability}
Theorems \ref{thm: LTI_Extension} and \ref{thm: LTI_Gram_PD} imply that Cases (2) and (4) are structurally observable in the sense of Definition 5 within any finite interval $0\leq t_0<t_1<\infty$, provided that at least one node exists on $\Omega$ at all times within the interval.   
\end{thm}
\emph{proof}:  As given in Section \ref{sec:Preliminaries}.1, The LTV systems defined in Cases (2) and (4) are structurally observable within the finite interval $0\leq t_0<t_1<\infty$ if a set of parameters governing the nonzero values of $\left(\mathbf{A},\mathbf{C}(t)\right)$, $\mathbf{p}(t)$, may be chosen such that the observability gramian shown in \eqref{eq: Obs_Gramian}\cite{chen_1999} is nonsingular:

\begin{equation}\label{eq: Obs_Gramian}
    \begin{split}
         W_O(t_0,t_1)&=\int_{t_0}^{t_1}e^{\mathbf{A}^\prime(t-t_0)}\mathbf{C}^\prime(t)\mathbf{C}(t)e^{\mathbf{A}(t-t_0)}dt\\
         &=e^{-\mathbf{A}^\prime t_0}\underbrace{\left(\int_{t_0}^{t_1}e^{\mathbf{A}^\prime t}\mathbf{C}^\prime(t)\mathbf{C}(t)e^{\mathbf{A}t}dt\right)}_{I_{LTV}(t_0,t_1)}e^{-\mathbf{A}t_0}
    \end{split}
\end{equation}

We subdivide $I_{LTV}(t_0,t_1)$ into a summation of integrals over adjacent, infinitesimal domains:

\begin{equation}\label{eq: LTV_Integral_Term}
    I_{LTV}(t_0,t_1)=\lim_{n\to\infty}\sum_{k=0}^{n-1}\int_{a(k)}^{b(k)}e^{\mathbf{A}^\prime t}\mathbf{C}^\prime(t)\mathbf{C}(t)e^{\mathbf{A}t}dt
\end{equation}

For ease of notation, we have defined $a(k)=\frac{k(t_1-t_0)}{n}+t_0$ and $b(k)=\frac{(k+1)(t_1-t_0)}{n}+t_0$.  In the limit as $n\to\infty$, $a(k)\to b(k)$ and the smoothly-varying $\mathbf{C}(t)$ reduces to the LTI matrix $\mathbf{C}_k$ within the $k^{th}$ infinitesimal integral domain:  

\begin{equation}\label{eq: LTV_Integral_Term_Reduced}
    I_{LTV}(t_0,t_1)=\lim_{n\to\infty}\sum_{k=0}^{n-1}\int_{a(k)}^{b(k)}e^{\mathbf{A}^\prime t}\mathbf{C}_k^\prime\mathbf{C}_ke^{\mathbf{A}t}dt
\end{equation}

\eqref{eq: LTV_Integral_Term_Reduced} may therefore be expressed as a summation of LTI observability gramians \eqref{eq: LTI_Gram}, valid within each infinitesimal domain:

\begin{equation}
    I_{LTV}(t_0,t_1)=\lim_{n\to\infty}\sum_{k=0}^{n-1}\underbrace{e^{\mathbf{A}^\prime a(k)}W_{O,LTI(k)}(a(k),b(k))e^{\mathbf{A}a(k)}}_{\mathbf{G}(k)}
\end{equation}
The matrix exponential $e^{\mathbf{A}t}$ and its transpose $\left(e^{\mathbf{A}t}\right)^\prime=e^{\mathbf{A}^\prime t}$ are nonsingular for all $t\in\mathbb{R}$ \cite{Godunov_1998}. Furthermore, provided that at least one node lays on $\Omega$ at all times in the interval $\left[t_0,t_1\right]$, a set of governing parameters for $\mathbf{A}$ and $\mathbf{C}_k$ may be chosen such that the symmetric gramian $W_{O,LTI(k)}(a(k),b(k))>0$ by Theorem \ref{thm: LTI_Gram_PD}.  This parameter set over the vanishing interval $(a(k),b(k))$ is denoted as $\mathbf{p}_k$.  Therefore by \cite{Horn_2013_LTV_cite} the symmetric matrix product $\mathbf{G}(k)>0$ for all $k\in\left\{0,1,2,\dots,n-1\right\}$. It follows then from \cite{Horn_2013_LTV_cite} that the summation of all $\mathbf{G}(k)$ is also PD, and therefore that the symmetric $I_{LTV}(t_0,t_1)>0$.  In the limit as $n\rightarrow\infty$, the sequence of $\mathbf{p}_k$ over the set of adjacent vanishing intervals defines the $\mathbf{p}(t)$ which allows for $I_{LTV}(t_0,t_1)>0$.  Therefore by \cite{Horn_2013_LTV_cite}, the symmetric product $ W_O(t_0,t_1)=e^{-\mathbf{A}^\prime t_0}I_{LTV}(t_0,t_1)e^{-\mathbf{A}t_0}>0$.  PD matrices are nonsingular, therefore $W_O(t_0,t_1)$ is nonsingular over any finite interval $\left[t_0,t_1\right]$.  Therefore the LTV systems defined in Cases (2) and (4) are structurally observable in the sense of Definition 5 because a $\mathbf{p}(t)$ exists such that $(\mathbf{A,C}(t))$ is observable on the interval $0\leq t_0<t_1<\infty$. $\blacksquare$

\begin{thm}\label{thm: LTV_Controllability}
Theorems \ref{thm: LTI_Extension}, \ref{thm: LTI_Gram_PD}, and \ref{thm: LTV_Observability} imply that Cases (3) and (4) are structurally controllable in the sense of Definition 5 within any finite interval $0\leq t_0<t_1<\infty$, provided that at least one node exists on $\Omega$ at all times within the interval.
\end{thm}
\emph{proof}:  As stated in Section \ref{sec:Preliminaries}.1, The LTV systems defined by Cases (3) and (4) are structurally controllable within the interval $0\leq t_0<t_1<\infty$ if a $\mathbf{p}(t)$ may be chosen such that the controllability gramian defined in \eqref{eq: LTV_Gram_Cont} \cite{chen_1999} is nonsingular.

\begin{equation}\label{eq: LTV_Gram_Cont}
    W_{C}(t_0,t_1)=e^{-\mathbf{A}t_0}\left(\int_{t_0}^{t_1}e^{\mathbf{A}t}\mathbf{B}(t)\mathbf{B}^\prime(t)e^{\mathbf{A}^\prime t}dt\right)e^{-\mathbf{A}^\prime t_0}
\end{equation}

Using this definition of controllability, the remainder of the proof proceeds similarly to that of Theorem \ref{thm: LTV_Observability}. $\blacksquare$

% \subsection{Structural controllability/observability with disconnected structures}

% Here, we expand on the limitations of predicted structural controllability/observability given in the previous section. PBF is particularly adept as making branching structures, which often results in segments that will be disconnected at some point in the build.  Fig. \ref{fig:hypo_nonobs} demonstrates a partially completed build in which segments of a branched structure are disconnected at the given layer, but will become connected in a future layer.  This build geometry enforces special conditions on the $\mathbf{A}$, $\mathbf{B}$, and $\mathbf{C}$ matrices of the linearized Hammerstein system.\par 
% $\mathbf{t}$ is divided into two parts, $\mathbf{t_1}$ and $\mathbf{t_2}$, which represent the temperatures of all nodes in the two disconnected structures. Since the two structures are thermally isolated and thus transfer no heat, $\mathbf{A}$ takes a block-diagonal structure as shown in Eq. \ref{eq:non_observeAC}.  Since structure 2 lies entirely beneath the powder, it contributes nothing to the system output and receives no system input for any linearization of the Hammerstein model.  Only the top surface of structure 1 receives input and constitutes the output.  As such, $\mathbf{B}$ and $\mathbf{C}$ take on the structures shown in \eqref{eq:non_observeAC}.   

% \begin{equation}
% \begin{aligned}
% \left[\begin{array}{c}
% \dot{\mathbf{t}}_1\\
% \hline
% \dot{\mathbf{t}}_2
% \end{array}\right]&=\underbrace{\left[\begin{array}{c|c}
% \mathbf{A}_1 & \mathbf{0}\\
% \hline
% \mathbf{0} & \mathbf{A}_2
% \end{array}\right]}_{\mathbf{A}}
% \left[\begin{array}{c}
% \mathbf{t}_1\\
% \hline
% \mathbf{t}_2
% \end{array}\right]+
% \underbrace{\left[\begin{array}{c}
% \mathbf{B}_1\\ \mathbf{0}\\
% \hline
% \mathbf{0}
% \end{array}\right]}_{\mathbf{B}}u\\
% \mathbf{y}&=\underbrace{\left[\begin{array}{cc|c}
% \mathbf{C}_1 & \mathbf{0} & \mathbf{0}
% \end{array}\right]}_{\mathbf{C}}\left[\begin{array}{c}
% \mathbf{t}_1\\
% \hline
% \mathbf{t}_2
% \end{array}\right]=\mathbf{y}_1+\mathbf{y}_2,
% \end{aligned}
% \label{eq:non_observeAC}
% \end{equation}

% \begin{cor}\label{cor:unobs}
% A thermal model \eqref{eq: LTI_System} that can be written in the form of \eqref{eq:non_observeAC} via row-rearrangement is neither structurally controllable nor observable.
% \end{cor}
% \emph{proof}: \eqref{eq:non_observeAC} may be viewed from the perspective of two disconnected networks $G(\mathbf{A}_1)$ and $G(\mathbf{A}_2)$ which may be analyzed separately.  The two networks have the dynamics shown below:

% \begin{equation}
%     \begin{split}
%         \dot{\mathbf{t}}_1&=\mathbf{A}_1\mathbf{t}_1+\begin{bmatrix}\mathbf{B}_1\\\mathbf{0}\end{bmatrix}\mathbf{u}\\
%         &\mathbf{y}_1=\left[\mathbf{C}_1,\mathbf{0}\right]\mathbf{t}_1
%     \end{split}\label{eq: ObservableSubSystem}
% \end{equation}

% \begin{equation}
%     \begin{split}
%         \dot{\mathbf{t}}_2&=\mathbf{A}_2\mathbf{t}_1+\mathbf{0}\mathbf{u}\\
%         &\mathbf{y}_2=\mathbf{0}\mathbf{t}_2
%     \end{split}\label{eq: ObservableSubSystem}
% \end{equation}

% Both $\mathbf{A}_1$ and $\mathbf{A}_2$ contain perfect matchings by Theorem 2, yet because structure 1 contains nodes on Face $\Omega$ of the build it retains structural controllability and observability.  In contrast, the construction of structure 2 as laying fully beneath the powder results in zero nodes on $\Omega$ and as such $G(\mathbf{A}_2)$ contains no nodes eligible for selection as driver/observer nodes.  Therefore, structure 2 is both structurally uncontrollable and unobservable.  This property is manifested by the $\mathbf{0}$ blocks which map the input-output relationships of state $\mathbf{t}_2$. The presence of an uncontrollable and unobservable subsystem in \eqref{eq:non_observeAC} renders the system uncontrollable and unobservable. $\blacksquare$   

% \subsection{Relative controllability and observability}
% The structural controllability/observability approach detailed in the previous subsections presents a simple ``yes/no'' verification to the question of controllability and observability.  Of practical interest are measures of \emph{relative} controllability/observability, which describe the relative ease with which input signals can control the system state and the ease with which system I/O can reconstruct the state, respectively.  To this end, we use the \emph{Hankel Singular Values} (HSVs) of Thermal Model \eqref{eq: LTI_System} \cite{chen_1999, Paganini_2000}:

% \begin{equation}
%     \Sigma=\{\sigma_i=\sqrt{\lambda_i\left(\mathbf{W}_c\mathbf{W}_o\right)}\geq0\:|\:\lambda_i\in\text{spec}(\mathbf{W}_c\mathbf{W}_o)\}\label{eq: HSVs}
% \end{equation}

% Here, $\mathbf{W}_c$ and $\mathbf{W}_o$ represent the controllability and observability gramians associated with Thermal Model \eqref{eq: LTI_System}, respectively. Each $\sigma_i$ represents the relative amount of energy transmitted to mode $i$ of the system from the input as well as the relative amount of energy mode $i$ contributes the system output.  $\sigma_i=0$ implies that the corresponding mode is either unobservable or uncontrollable, and values close to zero correspond to modes with negligible participation in system I/O dynamics (``weak'' HSVs).  We make an engineering decision that HSVs satisfying $\sigma_i\leq XXXXX\sigma_{max}$ are considered weak HSVs.  The proportion of weak HSVs with respect to the total count yields a measure of how readily the system may be controlled and observed.    

% \emph{Proof:}  Corollary \ref{cor:unobs} is proven via construction of the observability and controllability matrices, $\mathcal{O}$ and $\mathcal{C}$, respectively.  Given $\mathbf{A}_1\in\mathbb{R}^{n_1\times n_1}$ and $\mathbf{A}_2\in\mathbb{R}^{n_2\times n_2}$, $n_1+n_2 = n$, the observability matrix $\mathcal{O}$ equals

% \begin{equation}
% \mathcal{O}=\left[\begin{array}{c|c}
% \left[\begin{array}{cc}\mathbf{C}_1 & \mathbf{0}\end{array}\right] & \mathbf{0}\\
% \left[\begin{array}{cc}\mathbf{C}_1 & \mathbf{0}\end{array}\right]\mathbf{A}_1 & \mathbf{0}\\
% \vdots\\
% \left[\begin{array}{cc}\mathbf{C}_1 & \mathbf{0}\end{array}\right]\mathbf{A}_1^{n-1} & \mathbf{0}\\
% \end{array}
% \right],
% \end{equation}

% \noindent which has a maximum rank of $n_1<n$. Similarly, the controllability matrix $\mathcal{C}$ equals 

% \begin{equation}
% \mathcal{C}=\left[\begin{array}{cccc}
% \left[\begin{array}{c} \mathbf{B_1}\\\mathbf{0}\end{array}\right] & \left[\begin{array}{c} \mathbf{B_1}\\\mathbf{0}\end{array}\right]\mathbf{A_1}&\dots&\left[\begin{array}{c} \mathbf{B_1}\\\mathbf{0}\end{array}\right]\mathbf{A_1}^{n-1}\\
% \hline
% \mathbf{0}&\mathbf{0}&\dots&\mathbf{0}
% \end{array}\right]
% \end{equation}


% which has a maximum rank of $n_1<n$.$\blacksquare$  

% \begin{figure}[!tb]
% \centering
% \includegraphics[width=0.7\linewidth]{unobserve_hypothetical}
% \caption{\textbf{Observability of disconnected structures.}  In the hypothetical scenario here, the partially-built bridged structure has two legs, one in which there are observable and controllable state components and one in which the temperature measurements are either occluded by infrared opaque powder or out of the field of view (FOV). }
% \label{fig:hypo_nonobs}
% \end{figure}

% \subsection{Numerical evaluation of Controllability/Observability}
% As was discussed by the authors in \cite{Wood_2018}, the generally-unpredictable structure of thermal model \eqref{eq: LTI_System} complicates the prediction of controllability and observability outside of special cases such as that discussed in the previous section.  However, the standard tests for controllability and observability are of (e.g. the rank rest) are of little practical importance.  Thermal model \eqref{eq: LTI_System} is of an extremely large scale, with an order of $10^4$ nodes or higher, and may contain hundreds of `weakly' observable/controllable modes in which $\mathcal{O}$ and $\mathcal{C}$ barely pass the rank test.  Worse yet, numerical algorithms for computing matrix rank may be sensitive to a user specified tolerance, such as the Matlab \texttt{rank} and \texttt{obsvf} commands.\par 
% We continue to use the algorithm for numerically determining the unobservable subspace proposed by the authors in \cite{Wood_2018}.  For systems with non-defective $\mathbf{A}$, we avoid the previously-mentioned issues in detecting unobservable modes by placing the system in modal canonical form (MCF), and counting how many columns of the transformed $\mathbf{C}$ matrix, and how many rows of the transformed $\mathbf{B}$ matrix contain no nonzero values.  In MCF, each zero column of $\mathbf{C}$ corresponds to exactly one unobservable mode, and each zero row of $\mathbf{B}$ corresponds to exactly one uncontrollable mode, as noted in \cite{Brogan_1991}.\par   
% A similar MCF check exists for defective $\mathbf{A}$ if the system is transformed such that $\mathbf{A}$ is in Jordan Form.  Taking each Jordan block of transformed $\mathbf{A}$ to represent a ``mode'' of the system, the ``mode'' is controllable if the last row of transformed $\mathbf{B}$ associated with the block is nonzero, and it is observable if the first column of transformed $\mathbf{C}$ associated with the block is nonzero \cite{Brogan_1991}. The presence of zero rows/columns in the transformed $\mathbf{B}$/$\mathbf{C}$ corresponding to the block do not result in a loss of controllability/observability so long as these respective conditions hold. Unfortunately, the generalization of this technique to systems with defective $\mathbf{A}$ cannot be implemented, since numerically computing the Jordan form of $\mathbf{A}$ cannot be done reliably due to the problem being ill-conditioned \cite{Golub_1976}.\par 
% Implementing this technique on a digital computer naturally results in uncertainty as to what constitutes a ``zero'' element of the transformed $\mathbf{B}$ and $\mathbf{C}$, due to the finite precision of the machine. The \texttt{MATLAB} implementation of this algorithm considers any array element with absolute value less than \texttt{eps} $=2^{-52}$, the accuracy to whiche \texttt{MATLAB} can determine a deviation from the number 1, to be zero.  

% \subsection{Model order reduction via balanced realization}
% Thermal model \eqref{eq: LTI_System} was developed to mitigate the problem of model scale when attempting to represent PBF physics on the macroscale.  Even so, as noted previously, the size of the model presents numerous technical challenges and results in impractical computational burden.  Model order reduction (MOR) is necessary to reduce the impact of these issues.  We have chosen to perform MOR via \emph{residualization} \cite{Samar_1995,Skataric_2010}.\par
% The residualization algorithm begins by performing the linear state transformation $\mathbf{z}=\mathbf{Tt}$, which puts the system in its' balanced realization.  The user then selects the first $r$ (largest) Hankel Singular Values (HSVs) of the system, which are demonstrated in \eqref{eq:HSVs}.  Each HSV is $\sqrt{\lambda_i\left(\mathbf{W}_c\mathbf{W}_o\right)}$; $\lambda_i$ denotes the $i^{th}$ eigenvalue of a matrix, and $\mathbf{W}_c$ and $\mathbf{W}_o$ are the controllability and observability grammians, respectively.  

% \begin{equation}
% \Sigma=\textnormal{diag}\left(\sigma_1\geq\sigma_2\geq\ldots\geq \sigma_{n-\textnormal{Rank}\left(\mathcal{O}\right)}>0\right)
% \label{eq:HSVs}
% \end{equation}

% Partitioning the HSVs in this manner also partitions $\mathbf{z}$ into two groups: $\mathbf{z_1}\in\mathbb{R}^r$, which constitute the ``dominant'' modes in the system input/output dynamics, and $\mathbf{z_2}\in\mathbb{R}^{n-r}$, which constitute the negligible modes.  The partitioned system takes the form shown in Eq. 

% \begin{equation}
% \begin{split}
% &\begin{bmatrix}\mathbf{\dot{z}_1}\\\mathbf{\dot{z}_2}\end{bmatrix}=\begin{bmatrix}
% \mathbf{A_{11}}&\mathbf{A_{12}}\\\mathbf{A_{21}}&\mathbf{A_{22}}
% \end{bmatrix}\begin{bmatrix}
% \mathbf{z_1}\\\mathbf{z_2}\end{bmatrix}+\begin{bmatrix}
% \mathbf{B_{11}}\\\mathbf{B_{22}}
% \end{bmatrix}\mathbf{u}\\
% &\mathbf{y}=\begin{bmatrix}
% \mathbf{C_{11}}&\mathbf{C_{22}}
% \end{bmatrix}\begin{bmatrix}
% \mathbf{z_1}\\\mathbf{z_2}
% \end{bmatrix}
% \end{split}\label{eq: Partitioned_BalReal}
% \end{equation}

% The residualization algorithm assumes that the ``weak'' modes stored in $\mathbf{z_2}$ operate at quasi-steady state.  In other words, it assumes that on the time scales of interest, $\mathbf{\dot{z}_2}=0$. This assumption allows for the algebraic solution of $\mathbf{z_2}$, which reduces Eq. \ref{eq: Partitioned_BalReal} to the form shown in Eq. \ref{eq: Residualized_System}.

% \begin{equation}
% \begin{split}
% &\mathbf{\dot{z}_1}=\mathbf{A_rz_1}+\mathbf{B_ru}\\
% &\mathbf{y}=\mathbf{C_rz_1}+\mathbf{D_ru}\\
% &\mathbf{z_2}=-\mathbf{A_{22}}^{-1}\left(\mathbf{A_{21}z_1}+\mathbf{B_{22}u}\right)\\
% &\mathbf{A_r}=\mathbf{A_{11}-A_{12}A_{22}}^{-1}\mathbf{A_{21}}\\
% &\mathbf{B_r}=\mathbf{B_{11}-A_{12}A_{22}}^{-1}\mathbf{B_{22}}\\
% &\mathbf{C_r}=\mathbf{C_{11}-C_{22}A_{22}}^{-1}\mathbf{A_{21}}\\
% &\mathbf{D_r}=-\mathbf{C_{22}A_{22}}^{-1}\mathbf{B_{22}}
% \end{split}\label{eq: Residualized_System}
% \end{equation}

% With residualization, one only needs to solve $r$ coupled differential equations instead of $n$, and the original state $\mathbf{t}$ may be reconstituted during postprocessing by algebraically calculating $\mathbf{z_2}$ and performing the inverse transformation $\mathbf{t}=\mathbf{T}^{-1}\left[\mathbf{z_1}, \mathbf{z_2}\right]^T$.


==> results.tex <==
\section{SIMULATION RESULTS}\label{sec:results}

Tb. \ref{tb: System_stats} illustrates the results of the numeric observability check and the MOR procedure for both test parts.  It shows that the LTI systems corresponding to both test parts were unobservable, with an unobservable subspace of 45/1200 modes for Part (a) and 271/6831 modes for Part (b).  As such, the EnKF was incapable of forcibly driving the estimation error of all modes to zero.  Due to the detectability of all systems designed according to our approach, this unobservability did not produce divergent model error.  The table also shows the effectiveness of the model order reduction procedure.  Instead of running 100 parallel models with thousands of state components each, models on the order of ten state components were used.  

Fig. \ref{fig: ErrorComparison} plots the OL model error and CL estimation error for both test parts.  It reveals two important aspects of the filters' performance.  The addition of the EnKF reduced the model error in both test parts by approximately a factor of 2.5. Additionally, as Fig. \ref{fig: ErrorComparison} shows, the OL model error for Part (a) was unbounded.  This phenomena is due to the geometry of Part (a).  The Neumann boundary condition of Assumption \textbf{A2} trapped heat inside the ``arm'' of Part (a), therefore causing a monotonic temperature increase in that region.  The rate of increase was a function of the thermal diffusivity of the material being modeled, which was constructed to contain the maximum possible error.  This disparity in rates of temperature increase produced an unbounded OL model error signal.  As Fig. \ref{fig: ErrorComparison} shows, the filter stabilized this error such that it was bounded.   

Fig. \ref{fig: ErrorComparison} shows that both the OL model error and CL estimation error signals appeared to be strongly periodic for Part (b).  This phenomena is explained by Fig. \ref{fig: TestResults}, which illustrates the EnKF state estimation error for both test parts for sample time steps in the simulation.  One clearly observes from the figure that the region of maximum error closely ``followed'' the laser centerpoint.  This result was expected, given that the region nearest to the heat source produced the most extreme thermal response and thus deviated the furthest from the operating point of the linearization.  What appears to be periodic behavior in Fig. \ref{fig: ErrorComparison} is actually the superimposition of select few state components in Part (b) -- ie nodal temperatures corresponding to physical locations in the geometry -- experiencing a ``pulse'' of substantial error as the laser beam passed over them at staggered moments in time, before the heat diffused away and the regions decayed back to approximate ambient temperature with little error. 

Fig. \ref{fig: TestResults} also demonstrates that the CL estimation error oscillated about the laser point center.  The CL estimation error in the ``neck'' of Part (a) oscillated between positive and negative as the laser beam transitioned from close to far away from the $x=0$ plane.  Fig. \ref{fig: TestResults} shows that this tendency was also present in the CL estimation error in Part (b), with regions of positive and negative estimation error alternating radially outward from the laser centerpoint.  It is currently unknown what produces this wave-like pattern in the CL estimation error.  

\begin{table} [!b]
\centering
\caption{ Unobservable subspace $\mathcal{O}$ size and reduced system size for the test parts shown in Fig. \ref{fig: TestParts}}
\begin{tabular} {ccc}
\hline\hline
{Part}   & {$\mathcal{O}$ size} & {$n_{\text{reduced}}$}\\
\hline
{(a)} & {45} & {4} \\
{(b)}  & {272} & {33} \\
\hline\hline
\end{tabular}
\label{tb: System_stats}
\end{table}

\begin{figure*} [!tb]
\centering
\includegraphics[width=1.0\textwidth]{ErrorComparison_Fig.pdf}
\caption{Evolution of open loop model error (K) and closed loop estimation error (K) vs time (s) for Parts (a) and (b).  Every line represents the error signal for one state component (nodal temperature) in each respective LTI system.  Test part geometry shown in figure for reference.}
\label{fig: ErrorComparison}
\end{figure*} 

\begin{figure*} [!tb]
\centering
\includegraphics[width=1.0\textwidth]{test_results.pdf}
\caption{Demonstration of EnKF state estimation error for Parts (a) and (b) for sample time steps of the simulation.  Red dot represents the location of the laser beam centerpoint.}
\label{fig: TestResults}
\end{figure*}    


==> sim_study.tex <==
\section{CASE STUDIES DESCRIPTION}\label{sec:sim_setup}
Two case studies were conducted to assess the performance of the state estimator constructed in Sections \ref{sec:thermal_model}, \ref{sec:Controllability and Observability}, and \ref{sec:Estimator_design}.  These tests constitute a continuation of the work performed by the authors in \cite{Wood_2018}, in which data from assumed-accurate simulations were used in place of physical test parts.  We adopt the same basic ``virtual test'' procedure here.    

\subsection{Test procedures}
The simulated tests utilized the following procedure:

\begin{enumerate}
\item Construct a linearized state space model corresponding to test parts according to the procedures outlined in Section \ref{sec:thermal_model} and Fig. \ref{fig: GaussianDiscretization}.  The temperature along isothermal boundary $\Lambda$ was set to 0.  All test parts used material properties corresponding to Aluminum ore, tabulated in Tb. \ref{tb: MaterialProperties}.  Initial temperature was uniformly 0.  
\item Construct a heat conduction simulation in ANSYS utilizing the same test part geometry, mesh, and isothermal boundary, but with the full nonlinear treatment of the heat source.  Initial temperature was uniformly 0.  These simulations were used as surrogate ``true'' data, to test the amount of error incurred by the linearization process, $\mathbf{t}_k$.  
\begin{enumerate}
\item Tb. \ref{tb: MaterialProperties} shows that the material properties used to construct the LTI model and those used to construct the reference ANSYS simulation differed substantially. This was done to assess the effectiveness of the filter in purging modeling errors from the predicted $\mathbf{\hat{t}}$ in a worst-case scenario.  The material properties used to construct the reference ANSYS data were those corresponding to Aluminum at its' melting point, while those used to construct the linearized LTI model were those corresponding to Aluminum at room temperature, and therefore represent the maximum possible modeling error. 
\item A minor amount of process noise, visible in Fig. \ref{fig: TestLoading}, was added to the ANSYS laser data, to reflect Assumption \textbf{A5}.  This continuous-time noise had power equal to $1\times10^5$ mW for Part (a) and $2\times10^5$ mW for Part (b).    
\end{enumerate}  

\begin{table} [!b]
\centering
\caption{ Comparison of material properties used to construct LTI model data and reference ANSYS data for all test parts \cite{Marla_2014}}
\begin{tabular} {cccc}
\hline\hline
{Property }   & {LTI model} & {ANSYS data} & {Unit}\\
\hline
Thermal conductivity & {250} & {200} & {mW/mm-K}\\
Specific heat  & {$9\times10^8$} & {$1.248\times10^9$} & {mJ/tonne-K}\\
Density  & {$2.7\times10^{-9}$} & {$2.5\times10^{-9}$} & {tonne/mm$^3$}\\
\hline\hline
\end{tabular}
\label{tb: MaterialProperties}
\end{table}

\item Construct $\mathbf{u}_k$ for all test parts as Gaussian laser beams of a given power $P$ and variance $\sigma^2$ moving over the top surface $\Omega$ of the parts in a raster scanning path with average speed $v$, linearized according to Section \ref{sec:thermal_model}C and Fig. \ref{fig: GaussianDiscretization}.  This process is described in Section \ref{sec:sim_setup}C.  
\item Run the Ensemble Kalman Filter algorithm with the procedure described in Section \ref{sec:Estimator_design}C, using the constructed $\mathbf{u}_k$ as an input and using ANSYS data along surface $\Omega$ of the test parts from Step 2 as system measurements $\mathbf{y}_k$.  Recover temperature estimations $\mathbf{\hat{t}}_k$.
\begin{enumerate}
% \item The models were reduced by implicitly determining the size of $\mathbf{z}_1\in\mathbb{R}^r$, by grouping modes corresponding to HSVs with values less than $\left(\text{cutoff}\right)\sigma_{\text{max}}$ into $\mathbf{z}_1$ and the rest into $\mathbf{z}_2$.  The cutoff for Part (a) was 0.01 and the cutoff for Part (b) was 0.5.
\item Ensembles with $N=100$ members were used for both parts.
\item The continuous-time process noise power injected into $\mathbf{u}_k$ was $1\times10^5$ mW for Part (a) and $2\times10^8$ mW for Part (b), as shown in Fig. \ref{fig: TestParts}.  Increasing these noise powers tended to improve EnKF performance, since doing so increased the difference $\mathbf{z}^i_k-\mathbf{\bar{z}}_k$ for all ensemble members in \eqref{eq: SampleP}, therefore increasing the accuracy of computing $\mathbf{\bar{P}}^f_k$ for large N.  The continuous-time measurement noise power injected into $\mathbf{y}_k$ for both parts was 1 K.  
\end{enumerate}
\item Define the estimation error as $\text{Error}=\mathbf{t}_k-\mathbf{\hat{t}}_k$.  Plot and animate this error.
\item Run the LTI models corresponding to each test part in the open loop, according to \eqref{eq: LTI_System} and \eqref{eq: DiscreteSS_Model}.  Denote the open loop model predictions as $\mathbf{t}_{k,OL}$, and define the open loop model error as $\text{Error}_{OL}=\mathbf{t}_k-\mathbf{t}_{k,OL}$.  Comparisons between $\text{Error}$ and $\text{Error}_{OL}$ quantify the accuracy improvement produced by the filter.        
\end{enumerate}

\subsection{Test parts}

The two test parts utilized in this study are depicted in Fig. \ref{fig: TestParts}.  Information pertaining to the mesh and system size for these test parts is shown in Tb. \ref{tb: System_size}.  The slight discrepancy between node count and $n$ is due to temperature-constrained nodes along $\Lambda$ being removed from the system by ANSYS.    

\begin{figure} [!tb]
\centering
\includegraphics[width=0.5\textwidth]{TestParts.pdf}
\caption{Test parts used to conduct case studies.  Red arrows denote the basic path of the simulated laser beam. Part (a) referred to as the ``spool'' and Part (b) referred to as the ``coupon''}
\label{fig: TestParts}
\end{figure}   
   

\begin{table} [!b]
\centering
\caption{ Meshing information, system size $n$, and measurement count $p$ for test parts depicted in Fig. \ref{fig: TestParts}}
\begin{tabular} {cccccc}
\hline\hline
{Part}   & {Element size (mm)} & {Elements} & {Nodes} &{$n$} & {$p$}\\
\hline
{(a)} & {0.0333} & {540} & {1263} & {1200} & {63}\\
{(b)}  & {0.05} & {4861} & {8700} & {6831} & {1869}\\
\hline\hline
\end{tabular}
\label{tb: System_size}
\end{table}

\subsection{Test loading conditions}

Fig. \ref{fig: TestParts} illustrates the basic path of the laser beam across surface $\Omega$ for both test parts, as well as its nominal power $P$.  The laser power for both parts was computed according to the summed integral expression in \eqref{eq: HammersteinLoad}.  The time-varying laser centerpoints were calculated according to the expressions below.  \par 
The laser centerpoint $x(t)$ for Part (a) was calculated according to the expression:

\begin{equation}
x(t)=\frac{x_\text{max}-x_{\text{min}}}{2}\sin\left(\frac{v\pi}{x_\text{max}-x_{\text{min}}}t-\frac{\pi}{2}\right)+\frac{x_\text{max}+x_{\text{min}}}{2}\label{eq: PartACenterpoint}
\end{equation}

  Where $v=954$ $mm/s$, and $x_\text{max}$ and $x_\text{min}$ were taken from the part geometry as shown in Fig. \ref{fig: TestParts}. The end time of the simulation was set to be $t_\text{final}=4$ $ms$.  The variance of the beam was set to be $\sigma^2=0.01$.   

The laser centerpoint $\left\{x(t),y(t)\right\}$ for Part (b) was calculated according to the expression:

\begin{equation}
\begin{split}
&x(t)=\frac{x_\text{max}-x_{\text{min}}}{2}\sin\left(\frac{v\pi}{x_\text{max}-x_{\text{min}}}t-\frac{\pi}{2}\right)+\frac{x_\text{max}+x_{\text{min}}}{2}\\
&y(t)=\frac{y_\text{max}-y_\text{min}}{t_\text{final}}t+y_\text{min}
\end{split}\label{eq: PartBCenterpoint}
\end{equation}

Where $v=954$ $mm/s$, and $x_\text{max}$, $x_\text{min}$ $y_\text{max}$, and $y_\text{min}$ were taken from the part geometry as shown in Fig. \ref{fig: TestParts}.  The end time of the simulation was set to be $t_\text{final}=20$ $ms$.  The variance of the beam was set to be $\sigma^2=0.0225$.  Fig. \ref{fig: TestLoading} displays these loads for sample time steps in the simulation.  

\begin{figure*} [!tb]
\centering
\includegraphics[width=1.0\textwidth]{TestLoading.pdf}
\caption{Demonstration of simulated loading conditions for Parts (a), with magnification near the top surface for clarity, and Part (b).  Red contours indicate the noisy continuous Gaussian distribution used as input for ``true'' ANSYS-supplied data (not to scale), and the colored elements display the noise-free linearization of this loading according to the procedure outlined in Section \ref{sec:thermal_model}D and Fig. \ref{fig: GaussianDiscretization}.  This linearized loading was used as the input $\mathbf{u}_k$ for the Ensemble Kalman filter.}
\label{fig: TestLoading}
\end{figure*}    



==> state_estimator.tex <==
\section{STATE ESTIMATOR DESIGN}\label{sec:Estimator_design}

\subsection{Discretization of continuous-time model}
% This study utilized a Kalman filter to estimate the state of the reduced order model \eqref{eq: Residualized_System}, which required it to be implemented in discrete time.  The continuous-to-discrete time conversion of model \eqref{eq: LTI_System} for a discrete time step $\Delta t$ is shown in \eqref{eq: DiscreteSS_Model}: 
This study utilized a Kalman filter to estimate the state of Thermal Model \eqref{eq: LTI_System}, which required it to be implemented in discrete time.  The continuous-to-discrete time conversion of model \eqref{eq: LTI_System} for a discrete time step $\Delta t$ is shown in \eqref{eq: DiscreteSS_Model}: 
\begin{equation}
\begin{split}
&\mathbf{z}\left[k\right]=\mathbf{A_dz}\left[k-1\right]+\mathbf{B_du}\left[k\right]\\
&\mathbf{y}\left[k\right]=\mathbf{C_dz}\left[k\right]\\
&\mathbf{A_d}=e^{\mathbf{A}\Delta t}\approx \left(\mathbf{I}+\frac{1}{2}\Delta t\mathbf{A}\right)\left(\mathbf{I}-\frac{1}{2}\Delta t\mathbf{A}\right)^{-1}\\
&\mathbf{B_d}=\mathbf{A_r}^{-1}\left(\mathbf{A_d}-\mathbf{I}_r\right)\mathbf{B}\\
&\mathbf{C_d}=\mathbf{C}\\
\end{split}\label{eq: DiscreteSS_Model}
\end{equation}

% \begin{equation}
% \begin{split}
% &\mathbf{z}\left[k\right]=\mathbf{A_dz}\left[k-1\right]+\mathbf{B_du}\left[k\right]\\
% &\mathbf{y}\left[k\right]=\mathbf{C_dz}\left[k\right]+\mathbf{D_du}\left[k\right]\\
% &\mathbf{A_d}=e^{\mathbf{A_r}\Delta t}\approx \left(\mathbf{I_r}+\frac{1}{2}\Delta t\mathbf{A_r}\right)\left(\mathbf{I_r}-\frac{1}{2}\Delta t\mathbf{A_r}\right)^{-1}\\
% &\mathbf{B_d}=\mathbf{A_r}^{-1}\left(\mathbf{A_d}-\mathbf{I}_r\right)\mathbf{B_r}\\
% &\mathbf{C_d}=\mathbf{C_r}\\
% &\mathbf{D_d}=\mathbf{D_r}
% \end{split}\label{eq: DiscreteSS_Model}
% \end{equation}

The discretization scheme provided in \eqref{eq: DiscreteSS_Model} is based on the \emph{complete} discretization method given in \cite{Toth_2008} for a system with constant parameters.  The approximation of the matrix exponential $e^{\mathbf{A_r}\Delta t}$ in \eqref{eq: DiscreteSS_Model} is based on the Bilinear Transform as given in \cite{Franklin_1998}. 

\subsection{Stabilizability and detectability after discretization}
The discretization technique presented in the previous section was founded on the zero order hold (ZOH).  Here we show that following this procedure does not incur a loss of stabilizability or detectability in the system.
\begin{thm}
The eigenvalues of Thermal Model \eqref{eq: LTI_System} are real.
\end{thm}
\emph{proof}: In Thermal Model \eqref{eq: LTI_System}, the system $\mathbf{A}$ matrix is defined as $\mathbf{A}=-\mathbf{M}^{-1}\mathbf{K}$.  For simplicity of notation, define $\mathbf{H}=-\mathbf{M}^{-1}$, such that $\mathbf{A=HK}$, where $\mathbf{H}$ and $\mathbf{K}$ are symmetric, positive definite matrices.  As such, $\mathbf{H}$ has a unique positive definite, symmetric square root that satisfies the properties $\mathbf{H}^{1/2}\mathbf{H}^{1/2}=\mathbf{H}$, $\mathbf{H}^{1/2,T}=\mathbf{H}^{1/2}$ and $\mathbf{H}^{-1/2}\mathbf{H}^{1/2}=\mathbf{I}$ \cite{koeber_2006}. We conduct the following similarity transformation on $\mathbf{HK}$:

\begin{equation}
    \mathbf{HK}\rightarrow \mathbf{H}^{-1/2}(\mathbf{HK})\mathbf{H}^{1/2}=\mathbf{H}^{1/2}\mathbf{K}\mathbf{H}^{1/2}=\mathbf{H}^{1/2,T}\mathbf{K}\mathbf{H}^{1/2}\label{eq: DiscreteSimilarityCheck}
\end{equation}

As such, $\mathbf{HK}$ and $\mathbf{H}^{1/2}\mathbf{K}\mathbf{H}^{1/2}$ have the same eigenvalues.  Therefore, the eigenvalues of $\mathbf{HK}$ are real because $\mathbf{H}^{1/2}\mathbf{K}\mathbf{H}^{1/2}$ is symmetric as shown in \eqref{eq: RealEigenvalues}, and symmetric matrices have real eigenvalues \cite{golub_1996} $\blacksquare$.

\begin{equation}
    \left(\mathbf{H}^{1/2,T}\mathbf{K}\mathbf{H}^{1/2}\right)^T=\mathbf{H}^{1/2,T}\mathbf{K}^T\mathbf{H}^{1/2}=\mathbf{H}^{1/2,T}\mathbf{K}\mathbf{H}^{1/2}\label{eq: RealEigenvalues}
\end{equation}
\begin{cor}\label{cor: NoLossDiscretization}
Theorem 3 guarantees that \eqref{eq: DiscreteSS_Model} retains the stabilizability and detectability of Thermal Model \eqref{eq: LTI_System}.
\end{cor}
\emph{Proof}: Corollary \ref{cor: NoLossDiscretization} follows directly from the condition for retaining stabilizability/detectability after ZOH discretization specified in \cite{Kreisselmeier_1999, Middleton_1995} and the result of Theorem 3 $\blacksquare$.

\subsection{Ensemble Kalman filter (EnKF) implementation}
Effective implementation of a Kalman filter requires knowledge of the covariances pertaining to the process and measurement noise of the system under consideration.  The process noise covariance is denoted as $\mathbf{Q}$, and the measurement noise covariance is denoted as $\mathbf{R}$.  We intend to for model \eqref{eq: DiscreteSS_Model} to be implementable for arbitrary build layer geometry $V$ and under arbitrary external loading $q(\mathbf{\bar{v}},t)$.  These constraints make the prediction of $\mathbf{Q}$ intractable, while also limiting the utility of experimentally determining $\mathbf{Q}$ due to the near-infinite variety of allowable geometric and loading conditions.\par 
To overcome this limitation, we seek a means of approximating $\mathbf{Q}$ and $\mathbf{R}$ \emph{in-situ} from the measured data $\mathbf{y}$ and reconstructed state estimate $\mathbf{\hat{t}}$.  The \emph{Ensemble Kalman filter} detailed in \cite{Evensen_2003} provides the optimal means of accomplishing this goal.  What follows is a brief overview of the EnKF algorithm, readers interested in a complete description of EnKF theory should consult \cite{Evensen_2003}.\par 
Consider a discrete-time LTI model used to model some process:

\begin{equation}
\begin{split}
&\mathbf{z}_k=\mathbf{A_dz}_{k-1}+\mathbf{B_du}_k\\
&\mathbf{y}_k=\mathbf{C_dz}_k
\end{split}\label{eq: DiscreteProcessModel}
\end{equation}

The actual process modeled by \eqref{eq: DiscreteProcessModel} is depicted in \eqref{eq: DiscreteTimeModelNoFFD}, which contains (assumed independent) process noise $\mathbf{w}_k\sim\mathcal{N}(\mathbf{0,Q})$ and measurement noise $\mathbf{v}_k\sim\mathcal{N}(\mathbf{0,R})$:

\begin{equation}
\begin{split}
&\mathbf{z}_{k}=\mathbf{A_dz}_{k-1}+\mathbf{B_du}_k+\mathbf{w}_k\\
&\mathbf{y}_k=\mathbf{C_dz}_k+\mathbf{v}_k
\end{split}\label{eq: DiscreteTimeModelNoFFD}
\end{equation}

Accordingly, the EnKF treats the evolution of $\mathbf{z}_k$ as a random variable with some corresponding unknown true value $\mathbf{z}^t_k$. $\mathbf{z}^t_k$ would equal the value of $\mathbf{z}_k$ obtained from \eqref{eq: DiscreteProcessModel} if no noise were present.  The random variable $\mathbf{z}_k$ is distributed with the state error covariance $\mathbf{P}^f$:

\begin{equation}
\mathbf{P}^f_k=\mathbb{E}\left[(\mathbf{z}_k-\mathbf{z}^t_k)(\mathbf{z}_k-\mathbf{z}^t_k)^T\right]\label{eq: StateCovarianceDefinition}
\end{equation}

Similarly, the measurement $\mathbf{y}_k$ is treated as a random variable with some corresponding unknown,noise-free true value $\mathbf{y}^t_k$.  It is clear that $\mathbf{y}_k$ is distributed with measurement error covariance equal to $\mathbf{R}$:

\begin{equation}
\mathbf{R}=\mathbb{E}\left[(\mathbf{y}_k-\mathbf{y}^t_k)(\mathbf{y}_k-\mathbf{y}^t_k)^T\right]\label{eq: MeasurementCovarianceDefinition}
\end{equation}

As shown in \cite{Evensen_2003}, the EnKF defines an \emph{ensemble} of $N$ parallel instances of \eqref{eq: DiscreteTimeModelNoFFD}, denoted as $\mathbf{Z}_k=\left[\mathbf{z}^1_k,\mathbf{z}^2_k,\dots,\mathbf{z}^N_k \right]$, with corresponding measurement ensemble $\mathbf{Y}_k=\left[\mathbf{y}^1_k,\mathbf{y}^2_k,\dots,\mathbf{y}^N_k\right]$.  Each ensemble member $\mathbf{z}^i_k$, $\mathbf{y}^i_k$ is generated by running \eqref{eq: DiscreteTimeModelNoFFD} with independent instances of $\mathbf{w}_k$ and $\mathbf{v}_k$.  Therefore, $\mathbf{Z}_k$, $\mathbf{Y}_k$ collect $N$ samples of the random variables $\mathbf{z}_k$, $\mathbf{y}_k$.  By defining sample averages $\mathbf{\bar{z}}_k=\frac{1}{N}\sum\mathbf{z}^i_k$ and $\mathbf{\bar{y}}_k=\frac{1}{N}\sum\mathbf{y}^i_k$, one may construct the sample estimations of $\mathbf{P}^f_k$ and $\mathbf{R}$ as defined in \eqref{eq: StateCovarianceDefinition} and \eqref{eq: MeasurementCovarianceDefinition}, respectively:

\begin{align}
&\mathbf{\bar{P}}^f_k=\frac{1}{N-1}\sum_{i=1}^N(\mathbf{z}^i_k-\mathbf{\bar{z}}_k)(\mathbf{z}^i_k-\mathbf{\bar{z}}_k)^T\label{eq: SampleP}\\
&\mathbf{\bar{R}}_k=\frac{1}{N-1}\sum_{i=1}^N(\mathbf{y}^i_k-\mathbf{\bar{y}}_k)(\mathbf{y}^i_k-\mathbf{\bar{y}}_k)^T\label{eq: SampleR}
\end{align}

\cite{Evensen_2003} note that ensembles of size $N=100$ or greater estimate the true values of $\mathbf{P}^f_k$ and $\mathbf{R}_k$ to consistently acceptable accuracy.\par  
% Model order reduction is absolutely essential to avoid unreasonable computational burden when running several dozen concurrent models.\par 
Having defined $\mathbf{\bar{P}}^f_k$ and $\mathbf{\bar{R}}_k$, \cite{Evensen_2003} runs the standard Kalman filter update for every ensemble member:

\begin{equation}
\mathbf{\hat{z}}^i_k=\mathbf{z}^i_k+\mathbf{\bar{P}}^f_k\mathbf{C_d}^T\left(\mathbf{C_d\bar{P}}^f_k\mathbf{C_d}^T+\mathbf{\bar{R}}_k \right)^{\dagger}\left(\mathbf{y}^i_k-\mathbf{C_d}\mathbf{z}^i_k\right)\nonumber
\end{equation}

This process may be represented compactly by operating on the ensembles $\mathbf{Z}_k$ and $\mathbf{Y}_k$:

\begin{equation}
\mathbf{\hat{Z}}_k=\mathbf{Z}_k+\mathbf{\bar{P}}^f_k\mathbf{C_d}^T\left(\mathbf{C_d\bar{P}}^f_k\mathbf{C_d}^T+\mathbf{\bar{R}}_k \right)^{\dagger}\left(\mathbf{Y}_k-\mathbf{C_d}\mathbf{Z}_k\right)\label{eq: EnsembleFilter}
\end{equation}

The state estimate $\mathbf{\hat{z}}_k$ may be taken as the sample average of $\mathbf{\hat{Z}}_k$.  The updated ensemble estimates $\mathbf{\hat{Z}}_k$ are then fed into the ``predict'' step for the next time step in the algorithms' runtime, by substituting all $\mathbf{\hat{z}}^i_k$ into the RHS of their respective models as defined by \eqref{eq: DiscreteTimeModelNoFFD}.\par 

In order to better reflect the uncertainty in heat input within the PBF system stated in Assumption \textbf{A5}, we define an ensemble of inputs corresponding to $\mathbf{Z}_{1,k}$, $\mathbf{U}_k=\left[\mathbf{u}^1_k,\mathbf{u}^2_k,\dots,\mathbf{u}^N_k\right]$. Doing so makes the process input $\mathbf{u}_k$ stochastic via direct injection of the system process noise into the input for each ensemble member:

\begin{equation}
\begin{split}
&\mathbf{z}^i_{k}=\mathbf{A_d\hat{z}}^i_{k-1}+\mathbf{B_d}\left(\mathbf{u}_k+\mathbf{w}^i_k\right)\\
&\mathbf{y}^i_k=\mathbf{C_dz}^i_{k}+\mathbf{v}^i_k
\end{split}\label{eq: DiscreteTimeModelPlusNoise}
\end{equation}

By this definition, each ensemble member of $\mathbf{U}_k$ is defined as $\mathbf{u}^i_k=\mathbf{u}_k+\mathbf{w}^i_k$.  \eqref{eq: DiscreteTimeModelPlusNoise} can be expressed in more conventional form by rearrangement:

\begin{equation}
\begin{split}
&\mathbf{z}^i_{k}=\mathbf{A_d\hat{z}}^i_{k-1}+\mathbf{B_du}_k+\left(\mathbf{B_dw}^i_k\right)\\
&\mathbf{y}^i_k=\mathbf{C_d\hat{z}}^i_{k}+\mathbf{v}^i_k
\end{split}\nonumber 
\end{equation}

As shown in \cite{Tong_1990}, the multivariate normal distribution is closed under linear transformations and linear combinations, meaning that  $\mathbf{w}^i_k\sim\mathcal{N}(\mathbf{0,Q})$ produces $\mathbf{B_dw}^i_k\sim\mathcal{N}(\mathbf{0,B_dQB_d^T})$, and as such defining the process noise in this manner retains the assumption of Gaussian-distributed noise that underlies Kalman filter operation.\par 

% Our process model as described in \eqref{eq: DiscreteSS_Model} differs from the structure typically assumed for the operation of conventional Kalman filters \eqref{eq: DiscreteProcessModel}, due to the presence of direct feedthrough. Accounting for independent process noise $\mathbf{w}_k\sim\mathcal{N}\left(\mathbf{0,Q}\right)$ and measurement noise $\mathbf{v}_k\sim\mathcal{N}\left(\mathbf{0,R}\right)$, our stochastic process takes the form shown in in \eqref{eq: DiscreteTimeModelPlusNoise_Gen}. The subscript 1 attached to $\mathbf{z}_{1,k}$ indicates that the filter is estimating $\mathbf{z}_1$ of the reduced order system as defined in \eqref{eq: Residualized_System}, \eqref{eq: DiscreteSS_Model}.

% \begin{equation}
% \begin{split}
% &\mathbf{z}_{1,k}=\mathbf{A_dz}_{1,k-1}+\mathbf{B_du}_k+\mathbf{w}_k\\
% &\mathbf{y}_k=\mathbf{C_dz}_{1,k}+\mathbf{D_du}_k+\mathbf{v}_k
% \end{split}\label{eq: DiscreteTimeModelPlusNoise_Gen}
% \end{equation}

% We follow the modified Kalman filter architecture supplied in \cite{Gillijins_2007}, which acts to provide simultaneous unbiased minimum-variance estimates for the system input $\mathbf{u}_k$ and state $\mathbf{z}_{1,k}$ in the presence of systems with direct feedthrough.  To this end, we define an ensemble of inputs corresponding to $\mathbf{Z}_{1,k}$, $\mathbf{U}_k=\left[\mathbf{u}^1_k,\mathbf{u}^2_k,\dots,\mathbf{u}^N_k\right]$. \cite{Gillijins_2007} assumes that the values of all $\mathbf{u}^i_k$ are unknown.  We simulate this condition by making the process input $\mathbf{u}_k$ stochastic via direct injection of the system process noise into the input for each ensemble member:

% \begin{equation}
% \begin{split}
% &\mathbf{z}^i_{1,k}=\mathbf{A_d\hat{z}}^i_{1,k-1}+\mathbf{B_d}\left(\mathbf{u}_k+\mathbf{w}^i_k\right)\\
% &\mathbf{y}^i_k=\mathbf{C_dz}^i_{1,k}+\mathbf{D_d}\left(\mathbf{u}_k+\mathbf{w^i}_k\right)+\mathbf{v}^i_k
% \end{split}\label{eq: DiscreteTimeModelPlusNoise}
% \end{equation}

% By this definition, each ensemble member of $\mathbf{U}_k$ is defined as $\mathbf{u}^i_k=\mathbf{u}_k+\mathbf{w}^i_k$, and each ensemble member of $\mathbf{Y}_k$ is defined as $\mathbf{y}^i_k=\mathbf{C_dz}^i_{1,k}+\mathbf{D_du}^i_k+\mathbf{v}^i_k$.  Each member represents a sample from the randomly-distributed system inputs and measurements, respectively. This stochastic treatment of the process input reflects the uncertain nature of the PBF heat source, as stated in Assumption $\mathbf{A5}$. \eqref{eq: DiscreteTimeModelPlusNoise} can be expressed in more conventional form by rearrangement:

% \begin{equation}
% \begin{split}
% &\mathbf{z}^i_{1,k}=\mathbf{A_d\hat{z}}^i_{1,k-1}+\mathbf{B_du}_k+\left(\mathbf{B_dw}^i_k\right)\\
% &\mathbf{y}^i_k=\mathbf{C_d\hat{z}}^i_{1,k}+\mathbf{D_du}_k+\left(\mathbf{D_dw}^i_k+\mathbf{v}^i_k\right)
% \end{split}\nonumber 
% \end{equation}

% As shown in \cite{Tong_1990}, the multivariate normal distribution is closed under linear transformations and linear combinations, meaning that independent $\mathbf{w}^i_k\sim\mathcal{N}(\mathbf{0,Q})$ and $\mathbf{v}^i_k\sim\mathcal{N}(\mathbf{0,R})$ produce   $\mathbf{B_dw}^i_k\sim\mathcal{N}(\mathbf{0,B_dQB_d^T})$ and $(\mathbf{D_dw}^i_k+\mathbf{v}^i_k)\sim\mathcal{N}(\mathbf{0,D_dQD_d^T+R})$, and as such defining the process noise in this manner retains the assumption of Gaussian-distributed noise that underlies Kalman filter operation.\par 

% The filter architecture specified by \cite{Gillijins_2007} has three steps.  When combined with the EnKF architecture specified by \cite{Evensen_2003}, these steps take the following form:

% \begin{enumerate}
% \item \underline{Predict}.  Each ensemble member updates its ensemble values $\mathbf{z}^i_{1,k}$ according to \eqref{eq: DiscreteTimeModelPlusNoise}, using $\mathbf{u}^i_k$ as inputs, while collecting measurements collecting $\mathbf{y}^i_k$.  The ensemble is used to calculate sample estimates $\mathbf{\bar{P}}^f_k$ and $\mathbf{\bar{R}}_k$ according to \eqref{eq: StateCovarianceDefinition} and \eqref{eq: MeasurementCovarianceDefinition}, respectively.  
% \item \underline{Estimate input}.  Minimum-variance estimates for the ensemble member inputs are calculated by the following procedure:

% \begin{equation}
% \begin{split}
% &\mathbf{R}_1=\mathbf{C_d\bar{P}}^f_k\mathbf{C_d}^T+\mathbf{\bar{R}}_k\\
% &\mathbf{M}_k=\left(\mathbf{D_d}^T\mathbf{R}_1\mathbf{D_d}\right)^{\dagger}\mathbf{D_d}^T\mathbf{\bar{R}}^{\dagger}_k\\
% &\mathbf{\hat{U}}_k=\mathbf{M}_k\left(\mathbf{Y}_k-\mathbf{C_dZ}_{1,k}\right)
% \end{split}\label{eq: FFD_InputEstimation}
% \end{equation}

% \item \underline{Estimate state}.  Minimum-variance estimates for ensemble member state estimates $\mathbf{\hat{z}}^i_{1,k}$ are calculated according to an expression similar to \eqref{eq: EnsembleFilter}.  The procedure is outlined below:

% \begin{equation}
% \begin{split}
% &\mathbf{K}_k=\mathbf{\bar{P}}^f_k\mathbf{C_d}^T\mathbf{R}_1^{\dagger}\\
% &\mathbf{\hat{Z}}_{1,k}=\mathbf{Z}_{1,k}+\mathbf{K}_k\left(\mathbf{Y}_k-\mathbf{C_d}\mathbf{Z}_{1,k}-\mathbf{D_d\hat{U}}_k \right)
% \end{split}\label{eq: FFD_StateEstimation}
% \end{equation}
% \end{enumerate}

% In \eqref{eq: FFD_InputEstimation} and \eqref{eq: FFD_StateEstimation}, $\mathbf{M}_k$ and $\mathbf{K}_k$ are calculated with pseudoinverses because $\mathbf{\bar{R}}_k$ becomes singular if the number of measurements $p$ is greater than the number of ensemble members $N$, as noted in \cite{Evensen_2003}.  

\subsection{Filter algorithm summary}
\begin{itemize}
\item Construct a reduced order linearized model from the governing FEM-discretized heat transfer equation as done in Section \ref{sec:Controllability and Observability}D.
\item Express the model in discrete time as done in \eqref{eq: DiscreteSS_Model}.
\item Define initial temperature distribution throughout the part, express in terms of $\mathbf{z}_{k=0}$.
\item Define an ensemble of $N$ parallel instances of model \eqref{eq: DiscreteTimeModelPlusNoise}, each having ensemble members $\mathbf{z}^i_{k}$, $\mathbf{y}^i_k$, and $\mathbf{u}^i_k$.    
\end{itemize}

\noindent\texttt{for k=1:end of runtime}

\begin{itemize}
\item Determine $\mathbf{u}^i_k$ for all ensemble members according to $\mathbf{u}^i_k=\mathbf{u}_k+\mathbf{w}^i_k$, and run \eqref{eq: DiscreteSS_Model} for all ensemble members to generate all $\mathbf{z}^i_{1,k}$.  Ensemble member measurements $\mathbf{y}^i_k$ are constructed by corrupting the system measurement $\mathbf{y}_k$ with independent instances of white noise: $\mathbf{y}^i_k=\mathbf{y}_k+\mathbf{v}^i_k$.   Collect into ensembles $\mathbf{Z}_{k}$, $\mathbf{Y}_k$, and $\mathbf{U}_k$, respectively.
\item Compute $\mathbf{\bar{P}}^f_k$ and $\mathbf{\bar{R}}_k$ from \eqref{eq: SampleP} and \eqref{eq: SampleR}.  \item Estimate $\mathbf{\hat{Z}}_{1,k}$ according to \eqref{eq: EnsembleFilter}.
\item Construct estimated $\mathbf{\hat{z}}_{k}$ by taking the sample average of $\mathbf{\hat{Z}}_k$.
\end{itemize}
% \begin{itemize}
% \item Construct a reduced order linearized model from the governing FEM-discretized heat transfer equation as done in Section \ref{sec:Controllability and Observability}D.
% \item Express the model in discrete time as done in \eqref{eq: DiscreteSS_Model}.
% \item Define initial temperature distribution throughout the part, express in terms of $\mathbf{z}_{1,k=0}$.
% \item Define an ensemble of $N$ parallel instances of model \eqref{eq: DiscreteTimeModelPlusNoise}, each having ensemble members $\mathbf{z}^i_{1,k}$, $\mathbf{y}^i_k$, and $\mathbf{u}^i_k$.    
% \end{itemize}

% \noindent\texttt{for k=1:end of runtime}

% \begin{itemize}
% \item Determine $\mathbf{u}^i_k$ for all ensemble members according to $\mathbf{u}^i_k=\mathbf{u}_k+\mathbf{w}^i_k$, and run \eqref{eq: DiscreteSS_Model} for all ensemble members to generate all $\mathbf{z}^i_{1,k}$.  Ensemble member measurements $\mathbf{y}^i_k$ are constructed by corrupting the system measurement $\mathbf{y}_k$ with independent instances of white noise: $\mathbf{y}^i_k=\mathbf{y}_k+\mathbf{v}^i_k$.   Collect into ensembles $\mathbf{Z}_{1,k}$, $\mathbf{Y}_k$, and $\mathbf{U}_k$, respectively.
% \item Compute $\mathbf{\bar{P}}^f_k$ and $\mathbf{\bar{R}}_k$ from \eqref{eq: SampleP} and \eqref{eq: SampleR}.  
% \item Estimate $\mathbf{\hat{U}}_k$ according to \eqref{eq: FFD_InputEstimation}.
% \item Estimate $\mathbf{\hat{Z}}_{1,k}$ according to \eqref{eq: FFD_StateEstimation}.
% \item Construct estimated $\mathbf{\hat{z}}_{1,k}$ by taking the sample average of $\mathbf{\hat{Z}}_k$.
% \item Reconstruct $\mathbf{\hat{t}}_k$ according to the relationship between $\mathbf{\hat{z}}_{1,k}$, $\mathbf{\hat{z}}_{2,k}$ and $\mathbf{\hat{t}}_k=\mathbf{T}^{-1}\left[\mathbf{\hat{z}}_{1,k},\mathbf{\hat{z}}_{2,k}\right]^T$ outlined in \eqref{eq: Residualized_System}.
% \end{itemize}

\noindent\texttt{end}
